The Communication Complexity of Payment Computation

Let $(f,P)$ be an incentive compatible mechanism where $f$ is the social choice function and $P$ is the payment function. In many important settings, $f$ uniquely determines $P$ (up to a constant) and therefore a common approach is to focus on the design of $f$ and neglect the role of the payment function. Fadel and Segal [JET, 2009] question this approach by taking the lenses of communication complexity: can it be that the communication complexity of an incentive compatible mechanism that implements $f$ (that is, computes both the output and the payments) is much larger than the communication complexity of computing the output? I.e., can it be that $cc_{IC}(f)>>cc(f)$? Fadel and Segal show that for every $f$, $cc_{IC}(f)\leq exp(cc(f))$. They also show that fully computing the incentive compatible mechanism is strictly harder than computing only the output: there exists a social choice function $f$ such that $cc_{IC}(f)=cc(f)+1$. In a follow-up work, Babaioff, Blumrosen, Naor, and Schapira [EC'08] provide a social choice function $f$ such that $cc_{IC}(f)=\Theta(n\cdot cc(f))$, where $n$ is the number of players. The question of whether the exponential upper bound of Fadel and Segal is tight remained wide open. In this paper we solve this question by explicitly providing an $f$ such that $cc_{IC}(f)= exp(cc(f))$. In fact, we establish this via two very different proofs. In contrast, we show that if the players are risk-neutral and we can compromise on a randomized truthful-in-expectation implementation (and not on deterministic ex-post implementation) gives that $cc_{TIE}(f)=poly(n,cc(f))$ for every function $f$, as long as the domain of $f$ is single parameter or a convex multi-parameter domain. We also provide efficient algorithms for deterministic computation of payments in several important domains.

==> two_player_section.tex <==
	For every social choice function $f$, denote $P\colon V_1\times ...\times V_n \to \mathbb{R}^{n}$ as the payment scheme of the most efficient mechanism for $f$, i.e.  the one that satisfies $cc(f,P)=cc_{IC}(f)$. 
	Denote $P_{f}$ as the maximum number of prices for an alternative when using $P$.  Formally:
	\begin{equation*} \label{pfdefinition}
	P_{f} = \max_{i\in[N]} \hspace{0.5em} \max_{a\in \mathcal{A}} \hspace{0.5em} \big|\{p \hspace{0.5em} | \hspace{0.5em} \exists v\in V \hspace{0.5em} \text{s.t.} \hspace{0.5em} f(v)=a, \quad P_{i}(v)=p  \}\big|
	\end{equation*}
	\begin{theorem} \label{twoplayertheorem}
		Let $f$ be a social choice function for two players.
		Then:
		\begin{equation} \label{characterizationeq}
		\dfrac{cc(f)+ \log (P_{f})}{2} \le cc_{IC}(f)\le cc(f) + 2\log (P_{f})
		\end{equation}
	\end{theorem}
We stress Theorem \ref{twoplayertheorem} holds for all settings, multi-parameter as well as single-parameter. 
	\begin{proof}
		By definition, $cc_{IC}(f)\ge cc(f)$. 
		 Also, $cc_{IC}(f)\ge \log(P_{f}) $, because
		$cc_{IC}(f)\ge \log |\Ima (f,P)|\ge \log (P_{f})$. For the RHS of (\ref{characterizationeq}), denote the payment functions of players $1$ and $2$ with $P_1$ and with $P_2$, respectively. By the taxation principle, $P_1$ can be reformulated as a function of the alternative chosen and of $V_2$, and analogously $P_2$ is a function of the alternative chosen and of $V_1$. 
		\paragraph{} Denote $\Pi^f$ as the most efficient communication protocol of $f$. We will now describe a protocol for the mechanism. Fix types $v_1\in V_1, v_2\in V_2$. First,  the players run $\Pi^{f}(v_1,v_2)$, so they both know $f(v_{1},v_{2})=a$. By the above, once the alternative is known, player $1$ knows $P_2(a,v_{1})$ and player $2$ knows  $P_1(a,v_{2})$.   
		Hence, they just need to send to each other those payments, using at most $2\log(P_{f})$ bits. 
	\end{proof}
	\paragraph{Tightness.} If we drop $\log P_{f}$, there exists a social choice function for two players such that $cc_{IC}(f)=\exp(cc(f))$ (Theorem \ref{mostimportanttheorem}). Similarly, we can easily provide a function with one payment whose communication complexity (and thus the communication complexity of all its mechanisms)  is arbitrarily large. 
	\begin{definition} \label{disjscfdef}
		$f_k: V_1\times V_2\to \{a_0,a_1\}$.
		\newline 	\textbf{Input:} $v_{1}\in V_{1}$, $v_{2}\in V_{2}$ where $V_{1}=V_{2}=\{0,1,...,2^{k}-1\}$.
		\newline \textbf{Output:} $a_1$ if the bit representations of $v_{1},v_{2}$ are disjoint , $a_0$ otherwise. 
		\newline The public functions $w_{1},w_{2}:\{a_0,a_1\}\to \mathbb{R}$ are both constant zero, i.e. $w_{1}\equiv w_{2} \equiv 0$. 
	\end{definition}
	\paragraph{}Observe that players $1$ and $2$ are indifferent to the outcome of $f_k$, because their values $v_1\cdot w_{1}(a)$ and $v_2\cdot w_{2}(a)$ are a constant zero. Thus, they have no incentive to misreport their types, so a mechanism where the payments of both of them are always zero implements $f$. It is  also as efficient as possible, because computing the payments requires no communication at all.  
	 Hence, by definition $P_{f_k}=1$. 
	 In contrast, computing $f_k$ requires at least $k$ bits, as it can be trivially reduced to $DISJ_k$ which is known to require $k$ bits of communication \cite{ccbook}. 
%	 In contrast, $f_k$ is harder than the function $DISJ_{k}$ and it is well known that $CC(DISJ_{k})=\Omega(k)$ \cite{ccbook}.
	 Henceforth, $cc_{IC}(f_k)\ge cc(DISJ_k) \ge k$, so the gap between $P_{f_k}$ and $cc_{IC}(f_k)$ is arbitrarily large.
	\paragraph{} Observe that Theorem \ref{twoplayertheorem} is extremely similar to this  2-player characterization of mechanisms in \cite{dobzinski2016computational}. In order to state this characterization, we elaborate on the complexity measures for  mechanisms it uses.  Denote the set of menus that can be presented to player $i$ when using the mechanism $M$ with $M_{i}=\{\mathcal{M}_{v_{-i}}\hspace{0.25em}|\hspace{0.25em}v_{-i}\in V_{-i}\}$ and define  $tax(M)=\log (\max _{i} |M_{i}|)$. $tie(M)$ stands for the communication complexity of computing the allocation of  $M$, given that all players know the menu presented for every player $i$ according to $v_{-i}$.
		\begin{theorem} \cite{dobzinski2016computational} \label{shaharsthm}
			 Every $2-$player truthful mechanism $M$ for \textquote{rich enough} domains satisfies:
			\begin{equation*}
			\frac{tie(M)+ tax(M)}{2} \le cc(M)\le tie(M) + 2 \cdot tax(M)
			\end{equation*}
		\end{theorem}
		Theorems \ref{twoplayertheorem} and \ref{shaharsthm} differ in the following aspect. In Theorem \ref{twoplayertheorem}, we take an approach where we implicitly assume that mechanisms work by first computing the social choice function, and then computing payments. In contrast, Theorem \ref{shaharsthm} expresses a view where  the computation of a mechanism starts with displaying a menu of prices to each player, and afterwards selecting an alternative that maximizes utility for all players simultaneously. 
		\textcolor{orange}{This difference is actually prominent all over both papers. Should I write it here/in the introduction/at all?}
		\paragraph{} Notice that Theorem \ref{twoplayertheorem} characterizes $cc_{IC}(f)$ for all two-player functions. The LHS of (\ref{characterizationeq}) holds for all social choice functions. What about the RHS? Can we generalize the characterization beyond settings with two players? In other words, is it true that $cc_{IC}(f)\le poly(cc(f),\log(P_f))$ for all functions?
		 In Section \ref{polylogsec},  we answer this question in the negative.   
